Component-based Synthesis of Table Consolidation and Transformation Tasks from Examples

This paper presents an example-driven synthesis technique for automating a large class of data preparation tasks that arise in data science. Given a set of input tables and an out- put table, our approach synthesizes a table transformation program that performs the desired task. Our approach is not restricted to a fixed set of DSL constructs and can synthesize programs from an arbitrary set of components, including higher-order combinators. At a high-level, our approach performs type-directed enumerative search over partial pro- grams but incorporates two key innovations that allow it to scale: First, our technique can utilize any first-order specification of the components and uses SMT-based deduction to reject partial programs. Second, our algorithm uses partial evaluation to increase the power of deduction and drive enumerative search. We have evaluated our synthesis algorithm on dozens of data preparation tasks obtained from on-line forums, and we show that our approach can automatically solve a large class of problems encountered by R users.

==> background.tex <==
\section{Primer on Petri Nets} 

Since the remainder of this paper relies on basic knowledge about Petri nets, we first provide background on this topic.
%Readers who are already familiar with Petri nets are encouraged to skip ahead to the next section.

\subsection{Petri Net Definition}
A Petri net is a bipartite graph with two types of nodes: \emph{places}, which are drawn as circles, and \emph{transitions}, represented as solid bars (see Figure~\ref{fig:petri-ex}). Each place in a Petri net can contain a number of \emph{tokens}, which are drawn as dots and typically represent resources. A \emph{marking} (or \emph{configuration}) of a Petri net is a mapping from each place $p$ to the number of tokens at $p$. Transitions in the Petri net correspond to events that change the marking. In particular, incoming edges of a transition $t$ represent necessary conditions for $t$ to fire, and outgoing edges represent the outcome. For example, consider transition $T_1$ from Figure~\ref{fig:petri-ex}. A necessary condition for $T_1$ to fire is that there must be at least one token present at $P_1$, as the incoming edge to $T_1$ has weight $1$. %meaning that one token must be present at the source. 
Since the precondition of this transition is met, we say that $T_1$ is \emph{enabled}. If we fire transition $T_1$, we consume one token from place $P_1$ and produce one token at place $P_2$, as the outgoing edge of $T_1$ is also labeled with $1$. Figure~\ref{fig:petri-ex2} shows the result of firing $T_1$ at the configuration shown in Figure~\ref{fig:petri-ex}. Observe that transition $T_2$ is \emph{disabled} in both Figure~\ref{fig:petri-ex} and Figure~\ref{fig:petri-ex2} because there are fewer than two tokens at place $P_2$. 

\begin{definition}({\bf Petri net}) A Petri net is a five-tuple: 
\[ \pn = (P, T, E, W, M_0)\] where $P$ is a set of places, $T$ is a set of transitions, and $E \subseteq (P \times T) \cup (T \times P)$ is the set of edges (arcs). Finally, $W$ is a mapping from each edge $e \in E$ to a weight, and $M_0$ is the initial marking of $\pn$.
\end{definition}


\begin{figure}
\vspace{-0.2in}
\begin{center}
\includegraphics[scale=0.23]{pics/petri-ex.pdf}
\end{center}
\vspace{-0.1in}
\caption{A simple Petri net}\label{fig:petri-ex}
\vspace{-0.1in}
\end{figure}

\begin{figure}
\vspace{-0.1in}
\begin{center}
\includegraphics[scale=0.23]{pics/petri-ex2.pdf}
\end{center}
\vspace{-0.1in}
\caption{Result of firing $T1$ in Figure~\ref{fig:petri-ex}}\label{fig:petri-ex2}
\vspace{-0.1in}
\end{figure}

\begin{example}
Consider the Petri net shown in Figure~\ref{fig:petri-ex}. Here, we have $P = \{ P_1, P_2, P_3\}$ and $T = \{ T_1, T_2, T_3\}$. Let $e^*$ be the edge $P_2 \rightarrow T_2$. We have $W(e^*) = 2$, and $W(e) = 1$ for all other edges $e$ in $E$ (e.g., $P_1 \rightarrow T_1$). The initial marking $M_0$ assigns $P_1$ to 2, and all other places to $0$.
\end{example}



A \emph{run} (or \emph{trace}) of a Petri net $\pn$ is a sequence of transitions that are fired. For instance, some feasible runs of the Petri net shown in Figure~\ref{fig:petri-ex} include  $T_1, T_1, T_2$ and $T_1, T_1, T_2, T_3$. However, $T_1, T_2$ and $T_1, T_2, T_3$ are not feasible runs, since transition $T_2$ is disabled when there is a single token at place~$P_2$.

\subsection{Reachability and $k$-safety in Petri Nets}

A key decision problem about Petri nets  is \emph{reachability}: Given a Petri net $\pn$ with initial marking $M_0$ and a \emph{target marking} $M^*$, is it possible to reach $M^*$ by starting at $M_0$ and firing a sequence of transitions? For instance, consider the Petri net from Figure~\ref{fig:petri-ex} and the target marking $M^* = [P_1 \mapsto 0, P_2\mapsto 0, P_3 \mapsto 1]$. This marking is indeed reachable because we can get to marking $M^*$ by firing the sequence of transitions $T_1, T_1, T_2$. On the other hand, the marking $M^* = [P_1 \mapsto 0, P_2\mapsto 0, P_3 \mapsto 2]$ is not reachable from the initial configuration shown in Figure~\ref{fig:petri-ex}. The \emph{reachable state space} of a Petri net $\pn$, denoted $\reach(\pn)$, is the set of all markings that are reachable from the initial state. Given a Petri net $\pn$ and a target marking $M^*$, we say that a run  of $\pn$ is \emph{accepting} if it ends in $M^*$. 

Another important concept about Petri nets is the notion of \emph{k-safety}. A Petri net $\pn$ is said to be \emph{$k$-safe} if no place contains more than $k$ tokens for any marking in $\reach(\pn)$. For example, the Petri net shown in Figure~\ref{fig:petri-ex} is $2$-safe, since no place can contain more than 2 tokens in any configuration. However, if we modify this Petri net by adding a back edge from $T_1$ to $P_1$ (with an arc weight of 1), then the resulting Petri net is not $k$-safe for any $k$. 
As we will see later, the notion of $k$-safety plays an important role in the reachability analysis of Petri nets since the reachable state space $\reach(\pn)$ is bounded iff $\pn$ is $k$-safe.


==> intro_old.tex <==

\newcommand{\irule}[2]%
   {\mkern-2mu\displaystyle\frac{#1}{\vphantom{,}#2}\mkern-2mu} 
\newcommand{\irulelabel}[3]
{
\mkern-2mu
\begin{array}{ll}
\displaystyle\frac{#1}{\vphantom{,}#2} & #3
\end{array} 
\mkern-2mu
} 

\section{Introduction}

\begin{figure}[t]
\[
\begin{array}{lll}
{\rm Constant} \ c & := & {\rm True} \ | \ {\rm False} \ | \ {\rm null} \\
{\rm Table}   \ t & := & {\rm Table} \ t \\
{\rm Column}   \ l & := & {\rm Column} \ l \\
{\rm Expression} \ e & := & \sigma_\phi(e) \ | \ \pi(e) \ | \ e_1 \times e_2 \ | \ e_1 \cup e_2 \\
&& | \ f_{ag}(e) \ | \ f_{udf}(e)\\
{\rm Aggregator}  \ f_{ag} & := & f(e_1, e_2, ...), \\
&& f\in \{sum, avg, max, min\} \\
{\rm UserDefine}  \ f_{udf} & := & concat(e_1, e_2, ...) \ | \ substr(e_1) \ | \ ... \\
{\rm Operator}  \ op & := & > \ | < \ | = \ | \land \ | \ \lor \\
{\rm Predicate} \ \phi & := & v_1 \ op \ v_2 \ | \ \neg \phi \\
\end{array}
\]
\vspace{-0.2in}
\caption{Grammar of our core language}\label{fig:language}
\vspace{-0.1in}
\end{figure}


\begin{figure}[t]
\[
\begin{array}{lll}
{\rm Constraint \ Sketch} \ \comp & := & \constraint \\
{\rm Sketch}  \ \comp & := & \project_i(\sketch) \ | \select_{\constraint}(\comp) \ |  f(\comp) \\ 
&& | \comp_1 \times \comp_2 \ | \ \comp_1 \cup \comp_2 \\
\end{array}
\]
\caption{Sketch language}\label{fig:language}
\end{figure}

\begin{figure}[t]
\[
\begin{array}{lll}
\ Index & := & i \ | \ j \ | \ ... \\
\ Constraint & := & rowNum \ \star \ int \\  
                  && | \ colNum \ \star \ int \\  
                  && | \ cell(i,j) \ = \ int \\  
                  && | \ \constraint_1 \land \constraint_2 \ | \ \constraint_1 \lor \constraint_2 \\
                  && | \ i_1 \ \star \ i_2 \ | \ i_1 \ \star \ int \\
\ \star      & := & > \ | < \ | = \ | \geq \ | \ \leq \\
\end{array}
\]
\caption{Constraint language}\label{fig:language}
\end{figure}





\subsection{Commutative Laws}

% I have no idea how to properly format this.
\begin{enumerate}
\item $\sigma \circ \pi = \pi \circ \sigma$
\item $\sigma \circ \times > \times \circ (\sigma_1, \sigma_2)$
\item $\pi \circ \times > \times \circ (\pi_1, \pi_2)$
\item $a \circ \times$ is not a valid function
\item $\sigma \circ a = a$
\item $\pi \circ a = a$
\end{enumerate}

These laws show that we can ignore transformations of the form $\times \circ (\sigma_1, \sigma_2)$, $\times \circ (\pi_1, \pi_2)$, $a \circ \times$, $\sigma \circ a$, and $\pi \circ a$. Thus, all programs using just $\sigma$, $\pi$, $\times$, and $a$ take the recursive form:
\[
F = \sigma \circ \pi \circ (a \circ F \times a \circ F \times ... \times a \circ F)
\]

For laws 4 and 5, we ignore the trivial transformation to an empty table. Note that $A > B$ denotes that any transformation of form $B$ can also be represented in form $A$ (i.e. $A$ is more general than $B$).

\begin{comment} 
\subsection{Aggregate and Mapping Functions}

Functions that apply to an entire column (known as \textbf{aggregate functions}) are common in many database languages, yet they cannot be represented by Relational Algebra alone. This functions are often used in conjunction with some sort of grouping (like \texttt{GROUP BY} in SQL). Likewise, functions that modify each row in a table (we'll call these \textbf{mapping functions}) are also impossible to define with just Relational Algebra. To allow for these two types of functions, we include the following definitions.

% \theoremstyle{definition}
\begin{definition}{Aggregate Function}
An aggregate function is a function with the following structure:
\[
_\phi G _{f_1(A_1), f_2(A_2), ..., f_k(A_k)}
\]
where $\phi$ is a predicate that determines how rows are grouped, $f_i$ is a function that evaluates over a column, and $A_i$ is the column that $f_i$ should be evaluated over.
\end{definition}

\begin{definition}{Mapping Function}
An mapping function is a function with the following structure:
\[
H_{f_1(A_1^1, A_1^2, ..., A_1^{m_1}), ..., f_k(A_k^1, ..., A_k^{m_k})}
\]
where $f_i$ is a function that evaluates over $m_i$ values, and for each row, the $j^{th}$ argument for $f_i$ is in column $A_i^j$.
\end{definition}
\end{comment}

\subsection{Inference Rules}
We define our generic inference rules in figure \ref{fig:genconstraint}. In each rule, the given program evaluates to $\Phi$, the set of input constraints. The $\phi$ to the left of each $\vdash$ represents the output constraints of that program. $t^f_i$ defines a function that transforms the output constraints of $f$ to the input constraints of $f$'s $i^{th}$ input. Finally, for concrete table $T$, $\alpha(T)$ is the constraint system that describes $T$.
\begin{figure*}[t]
\[
\begin{array}{c}
\irule{
\begin{array}{c}
\phi_1' = t^f_1(\phi) \\ 
\phi_1' \vdash h_1 : \theta_1 \\
... \\
\Phi = \bigcup_i\theta_i \\
\end{array}
}
{\phi \vdash f(h_1, h_2, ...) : \Phi } 

\ \ \ \ \ \ \ \ 
\irule{
\begin{array}{c}
\\
\end{array}
}
{\phi \vdash input : \{\phi\} } 

\ \ \ \ \ \ \ \ 
\irule{
\begin{array}{c}
\alpha(T) \vdash f(h_1, h_2, ...) : \Phi \\
\end{array}
}
{\vdash f(h_1, h_2, ...) = T : \Phi } 

\end{array}
\]
\vspace{-0.1in}
\caption{Generic constraint rules}\label{fig:genconstraint}
\end{figure*}

\begin{figure*}[t]
\[
\begin{array}{c}
\irule{
\begin{array}{c}
\phi' = HAVOCROW(INTROWNUM((\phi)) \\ 
\phi' \vdash h_1 : \theta_1 \\
\Phi = \theta_1 \\
\end{array}
}
{\phi \vdash \sigma(h) : \Phi } 

\ \ \ \ \ \ \ \ 
\irule{
\begin{array}{c}
\phi' = HAVOCCOL(INTCOLNUM((\phi)) \\ 
\phi' \vdash h_1 : \theta_1 \\
\Phi = \theta_1 \\
\end{array}
}
{\phi \vdash \cup(h_1, h_2) : \Phi } 

\\\\
\ \ \ \ \ \ \ \ 
\irule{
\begin{array}{c}
\phi'_1 = UniqueRows(SubsetCols(0, s, \phi)) \\ 
\phi'_2 = UniqueRows(SubsetCols(s+1, end, \phi)) \\ 
\phi' \vdash h_1 : \theta_1 \\
\phi' \vdash h_2 : \theta_2 \\
\Phi = \{\theta_1, \theta_2\} \\
\end{array}
}
{\phi \vdash \times(h_1, h_2) : \Phi } 

\ \ \ \ \ \ \ \ 
\irule{
\begin{array}{c}
\phi'_1 = SubsetRows(0, s, \phi) \\ 
\phi'_2 = SubsetRows(s+1, end, \phi)) \\ 
\phi' \vdash h_1 : \theta_1 \\
\phi' \vdash h_2 : \theta_2 \\
\Phi = \{\theta_1, \theta_2\} \\
\end{array}
}
{\phi \vdash \cup(h_1, h_2) : \Phi } 

\end{array}
\]
\vspace{-0.1in}
\caption{Generic constraint rules. NOTE: UniqueRows replaces all repeated rows with a "?", effectively havocing that specific row. }\label{fig:genconstraint}
\end{figure*}




==> motivating-table.tex <==

\begin{figure*}
\centering
\begin{tabular}{ll}
\begin{tabular}{c c c c} 
     Input Table:\\
     \hline
     \rowcolor{lightgoldenrodyellow}
     course & year & class1 & class2 \\ [0.5ex] 
     \hline\hline
     \rowcolor{babyred}
     geometry & 2007 & 5 & 10\\
     \hline
     \rowcolor{babypurple}
     algebra & 2008 & 3 & 50\\
     \hline
     \rowcolor{babyred}
     geometry & 2007 & 5 & 17\\
     \hline
     \rowcolor{babypurple}
     algebra & 2008 & 6 & 17\\
     \hline
    \end{tabular}

    \hspace*{0.2in}
    \begin{tabular}{c c c c c} 
     Output Table:\\
     \hline
     \rowcolor{lightgoldenrodyellow}
     course & class1\_2007 & class2\_2007 & class1\_2008 & class2\_2008 \\ [0.5ex] 
     \hline\hline
     \rowcolor{babyred}
     geometry & 5 & 10 & 5 & 17\\
     \hline
     \rowcolor{babypurple}
     algebra & 3 & 50 & 6 & 17\\
     \hline
    \end{tabular}

    \end{tabular}
    \caption{Input-output tables for the motivating example.}\label{fig:motivating-table}
 \end{figure*}

==> synthesis-alg_old.tex <==
\setlength{\textfloatsep}{10pt}% Remove \textfloatsep
\begin{algorithm}[t]
\caption{Synthesis Algorithm}\label{alg:synthesis}
\begin{algorithmic}[1]
\vspace{0.05in}
\Procedure{Synthesize}{$k, \sketch, \tables, \comps, \Theta$}
\vspace{0.05in}
\State {\rm \bf Input:} Components $\comps$, Maximum $k$ components,
\State \ \ \ \ \ \ \ \ \ \ \ \ sketch with specs $\sketch$, input tables $\tables$
\State \ \ \ \ \ \ \ \ \ \ \ \ commutative law $\Theta$ 

%\State \ \ \ \ \ \ \ \ \ \ \ \ components $\comps$, and tests $\tests$
\State {\rm \bf Output:} Synthesized program or $\bot$ for failure
\vspace{0.05in}

\If{$k = 0$}
    \State $u$ := {\sc FindUnifier}($\sketch'$, $\tables$)
    \If{$u = \emptyset$}
        \State \Return $\bot$
    \EndIf
    \For{ $u_i \in u$ }
        \State $\prog$ := {\sc CompleteSketch}($u_i, \sketch$)
        \If{$\prog \neq \bot$}
            \State \Return $\prog$
        \EndIf
    \EndFor
    \State \Return $\bot$
\EndIf

\Comment e.g., {\sc subHoles}($\project_i(\sketch))=\sketch$
\For{ $(\comp_i, \constraint_i) \in$ {\sc subHoles}$(\sketch)$ }
    \For{ $f \in \comps$ }
        \State {\sc assume}($n$ = {\sc arity}($f$))
        \State $(\comp_1', ..., \comp_n')$ :=  {\sc FreshVar}($n$)
        \State $(\constraint_1', ..., \constraint_n')$ :=  {\sc Infer}($\constraint_i, f$)
        \State $\comp'$ :=  {\sc ReplaceHole}($\comp, i, 
        f(\comp_1':\constraint_1', ..., \comp_n': \constraint_n)$)
    \EndFor

    \State $\prog$ :=  {\sc Synthesize}($k-1, \comp':\constraint, \tables, \comps, \Theta$) 
    \If{$\prog \neq \bot$}
        \State \Return $\prog$
    \EndIf
\EndFor

\State \Return $\bot$
\EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\caption{FindUnifier}\label{alg:synthesis}
\begin{algorithmic}[1]
\vspace{0.05in}
\Procedure{FindUnifier}{$\sketch$, $\tables$}
\vspace{0.05in}
\State {\rm \bf Input:} Sketch with specifications $\sketch$,
\State \ \ \ \ \ \ \ \ \ \ \ \  input tables $\tables$
%\State \ \ \ \ \ \ \ \ \ \ \ \ components $\comps$, and tests $\tests$
\State {\rm \bf Output:} Mapping {\sc res} from sketch to input table
\vspace{0.05in}
\State {\sc res} := []
\For{ ($\comp_i, \constraint_i) \in $ {\sc subHoles}$(\sketch)$ }
    \For{ $u_j \in \tables$ }
        \If{{\sc SAT}$(\abs(u_j)\land \constraint_i)$}
            \State {\sc res}$[i]${\sc .insert}($u_j$)
        \EndIf
    \EndFor
\EndFor
\State \Return {\sc res}
\EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\caption{CompleteSketch}\label{alg:sketch}
\begin{algorithmic}[1]
\vspace{0.05in}
\Procedure{CompleteSketch}{$\sketch$, $\tables$}
\vspace{0.05in}
\State {\rm \bf Input:} Sketch with specifications $\sketch$,
\State \ \ \ \ \ \ \ \ \ \ \ \  input table $\tables$ 
%\State \ \ \ \ \ \ \ \ \ \ \ \ components $\comps$, and tests $\tests$
\State {\rm \bf Output:} A set $\prgTables$ of pair (programs,tables)  
\vspace{0.05in}

\If{{\sc isLeaf}($\sketch$)}
    \State $x$ := {\sc FreshVar}()
    \State \Return \{($x, \tables${\sc .front()})\}
\EndIf
{\sc assume}($\sketch = \comp:\constraint$)
{\sc assume}($\comp = \cst(\sketch_1, ..., \sketch_n)$)
\If{$\comp = \select (\sketch') \lor \comp = \project (\sketch') $}
    \State $\Theta$ := {\sc CompleteSketch}($\sketch'$, $\tables$)
    \For{ $(P,T) \in \Theta$ }
        \If{$\comp = \select (\sketch')$}
            \State $\preds$ := {\sc InferRows}($T', \constraint$)
        \Else
            \State $\preds$ := {\sc InferCols}($T', \constraint$)
        \EndIf
        \State $\prgTables$ := $\emptyset$
        \For{ $t \in \preds$ }
            \State $\prgTables${\sc .insert}($\cst_t(P), \cst_t(T)$)
        \EndFor
        \State \Return $\prgTables$
    \EndFor

\EndIf


\State $\Theta$ := {\sc CompleteSketch}($\sketch$, $\tables$)
\For{ $i \in [2,n]$ }
    \State $\Theta_i$ := {\sc CompleteSketch}($\sketch$, $\tables_i$)
    \State $\Theta$ := $\Theta \times \Theta_i$
\EndFor

\State $\Omega$ := $\{(\cst(\vec{P}), \cst(\vec{T})) | (\vec{P},\vec{T}) \in \Theta \land$ 
{\sc SAT}$(T=\cst(\vec{T}) \land \constraint) \}$

\State \Return $\prgTables$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{HavocRows}\label{alg:havoc_rows}
\begin{algorithmic}[1]
\vspace{0.05in}
\Procedure{HavocRows}{$\constraint$}
\vspace{0.05in}
\State {\rm \bf Input:} Constraint $\constraint$
\State {\rm \bf Output:} Modified constraint with row information havoced
\vspace{0.05in}

\State $I $ := $\{i \ | $ {\sc Cell} $(i, j)\in $ {\sc Atoms} $(\constraint)\}$
\State {\sc assume}($\constraint \implies \psi$) {\sc assume}($\psi = \bigwedge_{i\in I} i\ op\ j$)
\State $I' $ := {\sc FreshVars}$(|I|)$
\State $M $ := $I\mapsto I'$
\State $\constraint' $ := {\sc HRI}$(\constraint, M)$
\State \Return $\exists I.\constraint' \land I' \geq I \land \psi$

\EndProcedure

\Comment Not sure if you want to include HRI
\vspace{0.05in}
\Procedure{HRI}{$\constraint$, $M$}
\vspace{0.05in}
\State {\rm \bf Input:} Constraint $\constraint$
\State \ \ \ \ \ \ \ \ \ \ \ \  Mapping $M$ 
\State {\rm \bf Output:} Modified constraint

\If{$\constraint == (cell(i,j) = int)$}
	\State \Return $cell(M[i], j) = int$
\ElsIf{$\constraint == \constraint_1 \star \constraint_2$}
	\State \Return {\sc HRI}$(\constraint_1, M) \star ${\sc HRI}$(\constraint_2, M)$
\Else
	\State Return $\constraint$
\EndIf

\EndProcedure
\end{algorithmic}
\end{algorithm}

